Luban: Building Open-Ended Creative Agents via Autonomous Embodied Verification

Building open agents has always been the ultimate goal in AI research, and creative agents are the more enticing. Existing LLM agents excel at long-horizon tasks with well-defined goals (e.g., `mine diamonds' in Minecraft). However, they encounter difficulties on creative tasks with open goals and abstract criteria due to the inability to bridge the gap between them, thus lacking feedback for self-improvement in solving the task. In this work, we introduce autonomous embodied verification techniques for agents to fill the gap, laying the groundwork for creative tasks. Specifically, we propose the Luban agent target creative building tasks in Minecraft, which equips with two-level autonomous embodied verification inspired by human design practices: (1) visual verification of 3D structural speculates, which comes from agent synthesized CAD modeling programs; (2) pragmatic verification of the creation by generating and verifying environment-relevant functionality programs based on the abstract criteria. Extensive multi-dimensional human studies and Elo ratings show that the Luban completes diverse creative building tasks in our proposed benchmark and outperforms other baselines ($33\%$ to $100\%$) in both visualization and pragmatism. Additional demos on the real-world robotic arm show the creation potential of the Luban in the physical world.

==> sections/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All claims in the abstract and introduction are supported by the experiments in Sec \ref{sec:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please refer to the Sec \ref{sec:limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper is an application-oriented work rather than theoretical-oriented work, so this question is not applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The codes are included in Supplementary Materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The codes are included in Supplementary Materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please refer to the Sec \ref{sec:exp-1}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The error bars are plotted in the data analysis plots in Sec \ref{sec:exp-2} and Sec \ref{sec:exp-3}. Additionally, we use the Spearman correlation coefficients to demonstrate some conclusions in our paper, and we report the \emph{p-value} correspondingly.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In this work, our computing resources mainly involve accessing the OpenAI API, and we give an approximate cost in Appendix \ref{app:computational}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We make sure to preserve anonymity.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please refer to the Appendix \ref{app:broader-impacts}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assets in this work are credited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We release our codes and provide a brief \texttt{README} alongside the codes.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work involves human studies, please refer to Appendix \ref{app:human-study} for more details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The human studies of our work only involve the use of humans to evaluate Minecraft gameplay videos, which poses no potential risks to humans.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> sections/intro-new.tex <==
% \section{Introduction}

% Building open-ended agents that are grounded in the open world is always a long-term goal in the field of Artificial Intelligence (AI) research.
% Ideally, the agent should consume high-level abstract instructions and autonomously complete them in the environment without human intervention.
% Enabled by Large Language Models' (LLMs) \cite{gpt-4,lamma2} rich semantic knowledge and powerful reasoning capabilities, a series of open-ended agents based on LLM emerged recently.
% These LLM-based agents are targeted to physical (e.g., Robotics \cite{saycan,codeaspolicy,instruct2act,innerm}) or virtual (e.g., Minecraft Game \cite{Voyager,GITM,DEPS} and BabyAI \cite{babyai} Game \cite{hyvin}) environments, which first decompose instructions into action plans in the environment and then execute the action sequences to obtain feedback from the environment for grounding.

% % 这里的行文逻辑这样会不会更好点：
% % 1. straightforward task和creative task分别定义（主要是描述清楚closed和open goal state）
% % 2. creative task为啥更难/更有意义（比如更open）
% % 3. 现有的open-ended agent为啥只能做straightforward tasks而不能做后者
% % 4. 因此，总结问题就是open-ended agents for creative tasks
% However, existing LLM-based open-ended agents are limited to straightforward tasks in which agents consume clear instructions to take actions to reach a closed goal state (Figure \ref{fig:motivation} (a)).
% These agents rely on directly verifying (e.g. environment defined \cite{Voyager,GITM,DEPS} and autonomously proposed by agent \cite{hyvin}) the closed goal state to get the necessary feedback for grounding in the environment.
% For example, mining diamonds in Minecraft is a straightforward task. Despite diverse action sequences when mining diamonds, the agent can get feedback on the task's success by directly checking its inventory.
% Unfortunately, when facing open-ended creative tasks with abstract instructions and open goal states (Figure \ref{fig:motivation} (b)), existing agents fail to ground due to direct verification of the open state is infeasible.
% For example, building a house in Minecraft is a creative task. No direct verification of the target state of the openness house can be given.
% Therefore, building open-ended creative agents that can autonomously ground in environments remains a challenging issue.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/motivation.drawio.pdf}
%     \caption{(a) Agents for straightforward tasks v.s. (b) Luban agent for creative tasks.}
%     \label{fig:motivation}
% \end{figure}

% In this work, we propose the Luban agent, an open-ended creative building agent targeted in the open-world environment Minecraft, which relies on autonomous embodied verification to get feedback for grounding.
% As shown in Figure \ref{fig:motivation} (b), the key insight of the Luban agent is not to directly verify the open target state but to verify the shared functional set of them.
% Specifically, in the planning stage, the Luban agent first decomposes the open-ended creative building instructions into the subcomponents, then synthesizes Python code on a CAD modeling-based intermediate representation to build the subcomponents, and finally assembles them into a building.
% To reduce the open goal state space to make it feasible to verify the functional set, the Luban agent leverages the visual understanding capabilities of VLMs (i.e., \texttt{GPT-4V}) to perform visual verification subcomponents and assembly 3D models.
% In the execution stage, the Luban agent generates actions based on the 3D model obtained in the planning stage and executes them in the environment to construct the building.
% After construction, the Luban agent conducts pragmatic verification of the construction results, which autonomously synthesizes purposeful embodied actions to interact with the building based on the building's functional requirements and then summarizes and reflects on the action results and environment state to get feedback from the environment autonomously without human intervention.

% To evaluate the performance of our agent on open creative building tasks, we designed a small benchmark containing 5 Minecraft building tasks with diverse structural and functional requirements.
% Extensive human studies show that the Luban agent successfully ground in the environment to make pragmatic creations on open-ended creative building tasks and outperform the baselines of other methods in both multi-dimensional quality rating (similar to \cite{pku-creative-agent}) and Elo \cite{elo} rating.
% Moreover, the pass rate of action verification autonomously proposed by Luban agent is consistent with human assessment of functionality.
% Ablation study results demonstrate the effectiveness and necessity of the two-stage verification of the Luban agent.
% Finally, the demos in the embodied robotic arm environment demonstrated the potential of the Luban agent to perform open-ended creative tasks in the physical world.

% % In summary, we list the contributions of this work in the following three aspects:
% % \begin{itemize}
% %     \item We identify the difference between open-ended creative tasks and straightforward tasks and provide insights for verifying open-ended creative tasks, i.e., verify the shared functionality of open goal states. 
% %     \item Based on the insights, we proposed the open-ended creative agent, Luban, whose key is two-level autonomous embodied verification: visual verification and pragmatic verification.
% %     \item Extensive human studies show that the Luban agent surpasses baselines (i.e., quality and elo rating) on open-ended creative tasks, and the verification proposed by the agent is comparable to human. The ablation studies show the effectiveness and necessity of Luban's two-stage verification. Moreover, the robotic arm demos show the potential of Luban for application in the physical world.
% % \end{itemize}

% new ver
\section{Introduction}

Building open-ended agents that are grounded in the open world is always a long-term goal in the field of Artificial Intelligence (AI) research.
Ideally, the agent should consume high-level abstract instructions and autonomously complete them in the environment without human intervention.
Enabled by Large Language Models' (LLMs) \cite{gpt-4,lamma2} rich semantic knowledge and powerful reasoning capabilities, a series of open-ended agents based on LLM emerged recently, 
grounding in both physical (e.g., Robotics \cite{saycan,codeaspolicy,instruct2act,innerm}) or virtual (e.g., Minecraft Game \cite{Voyager,GITM,DEPS} and BabyAI \cite{babyai} Game \cite{sdground}) environments.

However, existing LLM-based open-ended agents are stuck in \psh{\textit{straightforward tasks}} where agents consume clear instructions and take actions to reach a \psh{well-defined ?} closed goal state (Figure \ref{fig:motivation} (a)), 
\psh{such as \sout{For example,}} the well-studied task of ``mining diamonds'' in Minecraft\psh{.\sout{ is a straightforward task.}}
Despite the agent \psh{experiencing diverse \sout{having diverse action}} trajectories when mining diamonds, they can finally reach a \psh{well-defined ?} closed goal state, i.e., having diamonds in their inventory.
Beyond straightforward tasks, \psh{\textit{creative tasks}} (Figure \ref{fig:motivation} (b)), another type of human-desired task mastered by agents, have abstract instructions and open goal states.
For example, building a house in Minecraft is a creative task. 
\psh{have abstract instructions to describe open goals without well-defined criteria, such as ``building a house'' in Minecraft}
\psh{\sout{The diverse action trajectories taken by the agent lead to open goal states, i.e., houses with different styles or designs.}}
\psh{The open goals of creative tasks bring great difficulties to agent design, because there are no formal standards to guide agent learning or evolution, i.e., diverse action trajectories lead to houses with different styles.}
% Existing straightforward task-oriented agents rely on directly verifying (e.g. environment defined \cite{Voyager,GITM,DEPS} and autonomously proposed by agent \cite{hyvin}) the closed goal state to get the necessary feedback for grounding in the environment, which makes them incompetent for creative tasks due to the unverifiability of the open goal state.
% Therefore, building open-ended creative agents that can autonomously ground in environments remains a challenging issue.
% \psh{Therefore, building open-ended agents that can autonomously ground open goal states in environments and complete creative tasks remains a challenging issue.}
Existing works have not fully explored creative task-oriented agents (only one early trial \cite{pku-creative-agent} without grounding \psh{only one early assessment work \cite{pku-creative-agent}}). 
\psh{\sout{and straightforward task-oriented agents are incapable of creative tasks.}}
\psh{Meanwhile, the straightforward task-oriented agents are obviously incapable of creative tasks, since they need to directly verify the closed goal state to ground the agent's behavior \cite{GITM,DEPS,hyvin}, which is impossible in creative tasks.}
\psh{\sout{
The reasoning is that these agents rely on directly verifying (e.g. environment defined \cite{Voyager,GITM,DEPS} and autonomously proposed by agent \cite{hyvin}) the closed goal state to get the necessary feedback for grounding in the environment, which makes them incompetent for creative tasks due to the unverifiability of the open goal state.
}}
Therefore, building open-ended agents that can autonomously ground open goal states in environments and complete creative tasks remains a challenging issue.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/motivation.drawio.pdf}
    \caption{(a) Agents for straightforward tasks v.s. (b) Luban agent for creative tasks.}
    \label{fig:motivation}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/motivation-2.jpg}
    \caption{(a) Agents for straightforward tasks v.s. (b) Luban agent for creative tasks.}
    \label{fig:motivation-2}
\end{figure}

In this work, we propose the Luban agent, an open-ended agent targeted for creative building tasks in the open-world environment Minecraft, which relies on autonomous embodied verification \psh{during planning and execution stages of the agent}to ground open goals.
As shown in Figure \ref{fig:motivation} (b), the key insight of the Luban agent is not to directly verify the open goal state but to propose and verify the shared functional set of them.
\psh{the key insight of the Luban agent is to autonomously propose and verify the well-defined shared functional set of open goals to solve creative tasks.}
Specifically, the Luban agent contains two-level progressive embodied verifications: (1) \textbf{visual verification in the planning stage} to reduce the open goal state space for the next level verification; (2) \textbf{pragmatic verification in the execution stage} that first propose the functional set, and then verify it in the environment by actions and states to ensure the functionalities.
For visual verification, Luban adopts CAD modeling programs as intermediate representations at the planning stage, which uses LLM first to decompose the open-ended creative building instructions into the subcomponents, then synthesize Python CAD modeling programs to build the subcomponents and assemble them into a building.
The Luban agent leverages the visual understanding capabilities of VLMs (i.e., \texttt{GPT-4V}) to perform visual verification subcomponents and assembly 3D models.
In the execution stage, the Luban agent generates actions based on the 3D model obtained in the planning stage and executes them in the environment to construct the building.
After construction, the Luban agent conducts pragmatic verification of the construction results, which autonomously synthesizes purposeful embodied actions to interact with the building based on the building's functional requirements and then summarizes and reflects on the action results and environment state to get feedback from the environment.

To evaluate the performance of our agent on open creative building tasks, we designed a benchmark containing 5 Minecraft building tasks with diverse structural and functional requirements.
Extensive human studies show that the Luban agent successfully ground in the environment to make pragmatic creations on open-ended creative building tasks and outperform the baselines of other methods in both multi-dimensional quality rating (similar to \cite{pku-creative-agent}) and Elo \cite{elo} rating.
Moreover, the pass rate of action verification autonomously proposed by Luban agent is consistent with human assessment of functionality.
Ablation study results demonstrate the effectiveness and necessity of the two-stage verification of the Luban agent.
Finally, the demos in the embodied robotic arm environment demonstrated the potential of the Luban agent to perform open-ended creative tasks in the physical world.

% In summary, we list the contributions of this work in the following three aspects:
% \begin{itemize}
%     \item We identify the difference between open-ended creative tasks and straightforward tasks and provide insights for verifying open-ended creative tasks, i.e., verify the shared functionality of open goal states. 
%     \item Based on the insights, we proposed the open-ended creative agent, Luban, whose key is two-level autonomous embodied verification: visual verification and pragmatic verification.
%     \item Extensive human studies show that the Luban agent surpasses baselines (i.e., quality and elo rating) on open-ended creative tasks, and the verification proposed by the agent is comparable to human. The ablation studies show the effectiveness and necessity of Luban's two-stage verification. Moreover, the robotic arm demos show the potential of Luban for application in the physical world.
% \end{itemize}

==> sections/introduction-old.tex <==
\section{Introduction}
% 1. open task? why important?

% 2. building satisfied human description is xx

% 3. current method: rl based -> llms based

% 4. key problem: accuracy, automated and scalable verification 

%% ours vs others
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/overview.drawio.pdf}
    \caption{Luban vs. Others}
    \label{fig:overview}
\end{figure}

% 从认知行为学的角度出发，说明开放任务探索的重要性
% 



\textbf{1. Problem definition:} %开放性agents是啥：
Open-ended is always the long-term goal for embodied AI agent research,
\sout{which means the agent can autonomously explore the environment, and try to complete abstractly described tasks without human-defined strict standards.}
which means the agent can accept abstract and free-form input task descriptions and autonomously complete them without human intervention.
The rapid advancement of large model technology has laid the groundwork for the study of open-ended agents.
The reasoning and planning abilities of large models allow agents to comprehend tasks described in natural language and to respond with appropriate actions.
Consequently, LMs-based agents are progressively becoming mainstream in the research of open-ended agents.
\sout{Specifically, we define three key criteria for open-ended embodied agents, open-ended unlimited tasks rather than pre-defined finite tasks, open-ended active learning rather than pre-defined passive learning, and they can pragmatically complete embodied tasks rather than give solutions in appearance.}

\textbf{2. Current methods:} %现在号称开放性要么是不开放（有标准），要么是假开放（外观开放）;
Many existing works claim that they have achieved open-ended agents.
However, these works all have varying degrees of limitations in terms of openness.
Some generative style works can give task solutions that only rely on language description, like GAI or creative agent, but they only meet the requirements in appearance. % which lack functional practicality in the embodied environment.
This is because the one-shot generation can hardly complete embodied tasks practically.
There are also some LMs-based agents trying to plan and execute in an iterative way to complete embodied tasks.
Nevertheless, they need carefully pre-trained skills or well-structured environment feedback, which violates the original intention of open-ended.
\sout{Some jobs focus only on the openness of tasks, but the learning process is passive and relies heavily on clearly defined criteria for task completion.
Deep reinforcement learning agents can transfer policies between similar tasks but rely on well-structured task rewards.
With the help of the generalizability of vision language models, recent large models-based agents can manipulate open-vocabulary objects following human instructions but still need passive training on the pre-collect dataset or explicit environment feedback.
There are also some generative style works that can give solutions that rely on language description.
However, they only meet the requirements in appearance, but lack functional practicality in the embodied environment. }

\textbf{3. Key problem + example:} %解释从外观开放到功能开放的难点;
\sout{Compared to giving a solution visually, pragmatically solving an embodied task in an open-ended way is undoubtedly more difficult.}
The key challenge of open-ended is how to enable the agent to accurately comprehend the implicit functional requirements within abstract descriptions in specific environments, without human assistance, thereby ensuring the pragmatical completion of tasks instead of merely providing ostensibly plausible solutions.
Taking the building tasks in the open-world game 'Minecraft' as an example,
giving an instruction ``build a bridge'' to make the bot build a bridge-like creation is relatively simple although the description is vague, since the solution has countless possibilities in appearance.
In construct, the instruction ``build a bridge to cross the river'' is hard to follow, since the task has implicit functional requirements but doesn't provide any clear definition or verification tools.
%\textbf{\TODO{summary key difficulties}}

\textbf{4. Motivation + ours method:}
Compared to AI agents, humans are good at handling such open-ended tasks.
With strong language understanding ability, rich knowledge reserve, and subjective initiative, humans can reason and formalize implicit functional requirements into clear standards, and actively keep trying and verifying until they successfully complete the task.
Inspired by humans' ability, we propose a multi-level self-verification vision language models-based agent framework, which is the first agent that can solve open-ended embodied tasks pragmatically.
The key insight is that through reasoning and self-validation at both the appearance and functional levels, intelligent agents can formalize and verify task descriptions to accomplish open-ended tasks within specific environments.

The details of our framework are shown in Figure \ref{fig_overview}.
With the help of the reasoning capacity of VLMs (like GPT-4 Vision), we designed a two-stage iterative framework to gradually refine, execute, and validate the given open-ended task in an autonomous way.
Consider building tasks in Minecraft, at the appearance planning level, we conduct subcomponent decomposition, generation, and assembling processes with CAD models as intermediate representations to autonomously create and verify the target building.
While at the functional execution level, to actually build and verify the functionality of the creation, we make the VLMs generate build and verification behavior codes separately in the Minecraft environment.
Then, after interacting with the environment by executing the code, we get the verification results and game state changes.
We use them as inputs to make the VLMs reflect whether the functionality meets the open-ended requirements, to drive next-step corrections.

\textbf{5.\TODO{Experiments:}}

==> sections/introduction.tex <==
% \section{Introduction}

% Building open-ended agents that are grounded in the open world is always a long-term goal in the field of Artificial Intelligence (AI) research.
% Ideally, the agent should consume high-level abstract instructions and autonomously complete them in the environment without human intervention.
% Enabled by Large Language Models' (LLMs) \cite{gpt-4,lamma2} rich semantic knowledge and powerful reasoning capabilities, a series of open-ended agents based on LLM emerged recently.
% These LLM-based agents are targeted to physical (e.g., Robotics \cite{saycan,codeaspolicy,instruct2act,innerm}) or virtual (e.g., Minecraft Game \cite{Voyager,GITM,DEPS} and BabyAI \cite{babyai} Game \cite{hyvin}) environments, which first decompose instructions into action plans in the environment and then execute the action sequences to obtain feedback from the environment for grounding.

% % 这里的行文逻辑这样会不会更好点：
% % 1. straightforward task和creative task分别定义（主要是描述清楚closed和open goal state）
% % 2. creative task为啥更难/更有意义（比如更open）
% % 3. 现有的open-ended agent为啥只能做straightforward tasks而不能做后者
% % 4. 因此，总结问题就是open-ended agents for creative tasks
% However, existing LLM-based open-ended agents are limited to straightforward tasks in which agents consume clear instructions to take actions to reach a closed goal state (Figure \ref{fig:motivation} (a)).
% These agents rely on directly verifying (e.g. environment defined \cite{Voyager,GITM,DEPS} and autonomously proposed by agent \cite{hyvin}) the closed goal state to get the necessary feedback for grounding in the environment.
% For example, mining diamonds in Minecraft is a straightforward task. Despite diverse action sequences when mining diamonds, the agent can get feedback on the task's success by directly checking its inventory.
% Unfortunately, when facing open-ended creative tasks with abstract instructions and open goal states (Figure \ref{fig:motivation} (b)), existing agents fail to ground due to direct verification of the open state is infeasible.
% For example, building a house in Minecraft is a creative task. No direct verification of the target state of the openness house can be given.
% Therefore, building open-ended creative agents that can autonomously ground in environments remains a challenging issue.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/motivation.drawio.pdf}
%     \caption{(a) Agents for straightforward tasks v.s. (b) Luban agent for creative tasks.}
%     \label{fig:motivation}
% \end{figure}

% In this work, we propose the Luban agent, an open-ended creative building agent targeted in the open-world environment Minecraft, which relies on autonomous embodied verification to get feedback for grounding.
% As shown in Figure \ref{fig:motivation} (b), the key insight of the Luban agent is not to directly verify the open target state but to verify the shared functional set of them.
% Specifically, in the planning stage, the Luban agent first decomposes the open-ended creative building instructions into the subcomponents, then synthesizes Python code on a CAD modeling-based intermediate representation to build the subcomponents, and finally assembles them into a building.
% To reduce the open goal state space to make it feasible to verify the functional set, the Luban agent leverages the visual understanding capabilities of VLMs (i.e., \texttt{GPT-4V}) to perform visual verification subcomponents and assembly 3D models.
% In the execution stage, the Luban agent generates actions based on the 3D model obtained in the planning stage and executes them in the environment to construct the building.
% After construction, the Luban agent conducts pragmatic verification of the construction results, which autonomously synthesizes purposeful embodied actions to interact with the building based on the building's functional requirements and then summarizes and reflects on the action results and environment state to get feedback from the environment autonomously without human intervention.

% To evaluate the performance of our agent on open creative building tasks, we designed a small benchmark containing 5 Minecraft building tasks with diverse structural and functional requirements.
% Extensive human studies show that the Luban agent successfully ground in the environment to make pragmatic creations on open-ended creative building tasks and outperform the baselines of other methods in both multi-dimensional quality rating (similar to \cite{pku-creative-agent}) and Elo \cite{elo} rating.
% Moreover, the pass rate of action verification autonomously proposed by Luban agent is consistent with human assessment of functionality.
% Ablation study results demonstrate the effectiveness and necessity of the two-stage verification of the Luban agent.
% Finally, the demos in the embodied robotic arm environment demonstrated the potential of the Luban agent to perform open-ended creative tasks in the physical world.

% % In summary, we list the contributions of this work in the following three aspects:
% % \begin{itemize}
% %     \item We identify the difference between open-ended creative tasks and straightforward tasks and provide insights for verifying open-ended creative tasks, i.e., verify the shared functionality of open goal states. 
% %     \item Based on the insights, we proposed the open-ended creative agent, Luban, whose key is two-level autonomous embodied verification: visual verification and pragmatic verification.
% %     \item Extensive human studies show that the Luban agent surpasses baselines (i.e., quality and elo rating) on open-ended creative tasks, and the verification proposed by the agent is comparable to human. The ablation studies show the effectiveness and necessity of Luban's two-stage verification. Moreover, the robotic arm demos show the potential of Luban for application in the physical world.
% % \end{itemize}

% new ver
\section{Introduction}

Building open-ended agents that are grounded in the open world is always a long-term goal in the field of Artificial Intelligence (AI) research.
Ideally, the agent should consume high-level abstract instructions and autonomously complete them in the environment without human intervention.
Enabled by Large Language Models' (LLMs) \cite{gpt-4,lamma2} rich semantic knowledge and powerful reasoning capabilities, a series of open-ended agents based on LLM emerged recently, 
grounding in both physical (e.g., Robotics \cite{saycan,codeaspolicy,instruct2act,innerm}) or virtual (e.g., Minecraft Game \cite{Voyager,GITM,DEPS} and BabyAI \cite{babyai} Game \cite{sdground}) environments.

However, existing LLM-based open-ended agents are stuck in \psh{\textit{straightforward tasks}} where agents consume clear instructions and take actions to reach a \psh{well-defined ?} closed goal state (Figure \ref{fig:motivation} (a)), 
\psh{such as \sout{For example,}} the well-studied task of ``mining diamonds'' in Minecraft\psh{.\sout{ is a straightforward task.}}
Despite the agent \psh{experiencing diverse \sout{having diverse action}} trajectories when mining diamonds, they can finally reach a \psh{well-defined ?} closed goal state, i.e., having diamonds in their inventory.
Beyond straightforward tasks, \psh{\textit{creative tasks}} (Figure \ref{fig:motivation} (b)), another type of human-desired task mastered by agents, have abstract instructions and open goal states.
For example, building a house in Minecraft is a creative task. 
\psh{have abstract instructions to describe open goals without well-defined criteria, such as ``building a house'' in Minecraft}
\psh{\sout{The diverse action trajectories taken by the agent lead to open goal states, i.e., houses with different styles or designs.}}
\psh{The open goals of creative tasks bring great difficulties to agent design, because there are no formal standards to guide agent learning or evolution, i.e., diverse action trajectories lead to houses with different styles.}
% Existing straightforward task-oriented agents rely on directly verifying (e.g. environment defined \cite{Voyager,GITM,DEPS} and autonomously proposed by agent \cite{hyvin}) the closed goal state to get the necessary feedback for grounding in the environment, which makes them incompetent for creative tasks due to the unverifiability of the open goal state.
% Therefore, building open-ended creative agents that can autonomously ground in environments remains a challenging issue.
% \psh{Therefore, building open-ended agents that can autonomously ground open goal states in environments and complete creative tasks remains a challenging issue.}
Existing works have not fully explored creative task-oriented agents (only one early trial \cite{pku-creative-agent} without grounding \psh{only one early assessment work \cite{pku-creative-agent}}). 
\psh{\sout{and straightforward task-oriented agents are incapable of creative tasks.}}
\psh{Meanwhile, the straightforward task-oriented agents are obviously incapable of creative tasks, since they need to directly verify the closed goal state to ground the agent's behavior \cite{GITM,DEPS,hyvin}, which is impossible in creative tasks.}
\psh{\sout{
The reasoning is that these agents rely on directly verifying (e.g. environment defined \cite{Voyager,GITM,DEPS} and autonomously proposed by agent \cite{hyvin}) the closed goal state to get the necessary feedback for grounding in the environment, which makes them incompetent for creative tasks due to the unverifiability of the open goal state.
}}
Therefore, building open-ended agents that can autonomously ground open goal states in environments and complete creative tasks remains a challenging issue.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/motivation.png}
    \caption{(a) Agents for straightforward tasks v.s. (b) Luban agent for creative tasks.}
    \label{fig:motivation}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/motivation-2.jpg}
    \caption{(a) Agents for straightforward tasks v.s. (b) Luban agent for creative tasks.}
    \label{fig:motivation-2}
\end{figure}

In this work, we propose the Luban agent, an open-ended agent targeted for creative building tasks in the open-world environment Minecraft, which relies on autonomous embodied verification \psh{during planning and execution stages of the agent}to ground open goals.
As shown in Figure \ref{fig:motivation} (b), the key insight of the Luban agent is not to directly verify the open goal state but to propose and verify the shared functional set of them.
\psh{the key insight of the Luban agent is to autonomously propose and verify the well-defined shared functional set of open goals to solve creative tasks.}
Specifically, the Luban agent contains two-level progressive embodied verifications: (1) \textbf{visual verification in the planning stage} to reduce the open goal state space for the next level verification; (2) \textbf{pragmatic verification in the execution stage} that first propose the functional set, and then verify it in the environment by actions and states to ensure the functionalities.
For visual verification, Luban adopts CAD modeling programs as intermediate representations at the planning stage, which uses LLM first to decompose the open-ended creative building instructions into the subcomponents, then synthesize Python CAD modeling programs to build the subcomponents and assemble them into a building.
The Luban agent leverages the visual understanding capabilities of VLMs (i.e., \texttt{GPT-4V}) to perform visual verification subcomponents and assembly 3D models.
In the execution stage, the Luban agent generates actions based on the 3D model obtained in the planning stage and executes them in the environment to construct the building.
After construction, the Luban agent conducts pragmatic verification of the construction results, which autonomously synthesizes purposeful embodied actions to interact with the building based on the building's functional requirements and then summarizes and reflects on the action results and environment state to get feedback from the environment.

To evaluate the performance of our agent on open creative building tasks, we designed a benchmark containing 5 Minecraft building tasks with diverse structural and functional requirements.
Extensive human studies show that the Luban agent successfully ground in the environment to make pragmatic creations on open-ended creative building tasks and outperform the baselines of other methods in both multi-dimensional quality rating (similar to \cite{pku-creative-agent}) and Elo \cite{elo} rating.
Moreover, the pass rate of action verification autonomously proposed by Luban agent is consistent with human assessment of functionality.
Ablation study results demonstrate the effectiveness and necessity of the two-stage verification of the Luban agent.
Finally, the demos in the embodied robotic arm environment demonstrated the potential of the Luban agent to perform open-ended creative tasks in the physical world.

% In summary, we list the contributions of this work in the following three aspects:
% \begin{itemize}
%     \item We identify the difference between open-ended creative tasks and straightforward tasks and provide insights for verifying open-ended creative tasks, i.e., verify the shared functionality of open goal states. 
%     \item Based on the insights, we proposed the open-ended creative agent, Luban, whose key is two-level autonomous embodied verification: visual verification and pragmatic verification.
%     \item Extensive human studies show that the Luban agent surpasses baselines (i.e., quality and elo rating) on open-ended creative tasks, and the verification proposed by the agent is comparable to human. The ablation studies show the effectiveness and necessity of Luban's two-stage verification. Moreover, the robotic arm demos show the potential of Luban for application in the physical world.
% \end{itemize}
